Hybrid Design of Multiplicative Watermarking for Defense Against Malicious Parameter Identification

Watermarking is a promising active diagnosis technique for detection of highly sophisticated attacks, but is vulnerable to malicious agents that use eavesdropped data to identify and then remove or replicate the watermark. In this work, we propose a hybrid multiplicative watermarking (HMWM) scheme, where the watermark parameters are periodically updated, following the dynamics of the unobservable states of specifically designed piecewise affine (PWA) hybrid systems. We provide a theoretical analysis of the effects of this scheme on the closed-loop performance, and prove that stability properties are preserved. Additionally, we show that the proposed approach makes it difficult for an eavesdropper to reconstruct the watermarking parameters, both in terms of the associated computational complexity and from a systems theoretic perspective.

==> Sections/Draft.tex <==

Cyber-physical systems have risen from the increased presence of distributed sensing, computational and communication technologies in industrial settings. In CPSs, local sensors capture the state of local plants and send it to the remote control center. The control center generates control signals based on the measurements received and sends the control signals to the plants. The integration of distributed components --- plants, sensors, controllers --- enables operators to control plants from far away and utilize cloud computation resources to execute more complex control algorithms, which improve the capability of controlling large-scale systems. Because of the advantages of the CPSs, more and more infrastructures have started to use CPSs design methods to design their control systems, such as industrial manufacturing systems, medical healthcare systems, and power management systems. 

%% security problem of CPSs + attack story
The wide application of CPSs in safety-critical infrastructures puts forward high requirements for security. However, the current design methods of the CPSs have security defects. For example, the network layer of the CPSs mainly uses protocols in industrial control systems such as Modbus \citep{alguliyevCyberphysicalSystemsTheir2018}, which meet the real-time requirements of CPSs but lack security mechanisms \citep{xuReviewCyberVulnerabilities2017}. These defections make CPSs vulnerable to malicious attacks. Attackers can easily access the communication network and modify the sensor or control signals, thus ruining the original plant without being detected, such as the well-known Stuxnet worm program. Such attacks on CPSs will cause disastrous effects and economic loss.

%% current solution for security
% 1. cryptography not suitable
% 2. examples of security solution
% 3. passive detection + active detection
% 4. but under system-identification attack
% 5. ways to deal with system identification attack
% 6. pseudo-random generator problem

% cryptography not suitable
\emph{The design of securing Cyber-physical Systems is imperative}. A direct way is to encrypt signals using cryptography tools such as RSA encryption. However, most cyber-physical systems require low feedback delay. Processing advanced cryptography algorithms on sensors, or actuators can be time-consuming. Furthermore, it is unrealistic to upgrade all legacy components. The requirements and restrictions of CPSs demand lightweight solutions. 

% passive detection methods
One popular research direction is \textbf{passive detection methods} \cite{dinhvuApplyingFaultDetectors2016, shoukryEventTriggeredStateObservers2016a, liAttackDetectionCyberPhysical2018}. Passive detection methods detect malicious modifications or recover actual data using components in the original systems. These methods do not actively change the plant's or controller's structure. However, the usage of passive detection methods is strict. For example, the method in \cite{shoukryEventTriggeredStateObservers2016a} is effective only if at least a certain number of sensors is safe. Additionally, an attacker with perfect system knowledge can design a malicious covert attack sequence, which will destroy the system but remain invisible. 

% active detection methods introduction
\textbf{Active detection methods} are another trend of attack detection methods \cite{moSecureControlReplay2009, miaoCodingSensorOutputs2014, weerakkodyActiveDetectionExposing2017, ferrariDetectionIsolationReplay2017b, guoOutputCodingBasedDetectionScheme2021, ghaderiBlendedActiveDetection2021}. Unlike passive detection methods, active detection methods will add some secret structures to the system and detect malicious attacks according to the property of the secret structures. 

% review of the active detection methods
% additive watermarking method
In \cite{moSecureControlReplay2009}, the author proposes the additive watermarking method. In the additive watermarking method, the defender adds some private zero-mean random value to the controller output and tries to detect the residual change under different attacks. The additive watermarking cannot detect additive covert attacks and will cause performance loss to the system.

% coding matrix method
In \cite{miaoCodingSensorOutputs2014}, the authors propose to encode the sensor measurement by a private matrix to detect data deception attacks. Because the controller side will decode the signal can with the inverse matrix, the method will not cause performance loss. However, the proposed method is only available for MIMO systems.

% moving target method
In \cite{weerakkodyActiveDetectionExposing2017}, the author adds an auxiliary system parallel to the original plant.
At each timestamp, the plant and controller sides will generate a group of parameters for the auxiliary system. If the attacker cannot access the parameter of the auxiliary system, it cannot design stealthy attacks.

% multiplicative watermarking method
The author proposes a multiplicative watermarking method in \cite{ferrariDetectionIsolationReplay2017b}. The multiplicative watermarking uses a stateful transformation to encode the sensor measurement and decode it on the controller side. The multiplicative watermarking will not cause performance loss and will be helpful for detecting malicious attacks if the parameter of the watermarking generator is unknown to the attacker.

% when identified -> easy to be broken
% some methods consider this part -> introduce extra risk or hard to implement
Because active detection methods rely on the property of the secret structure, they can be broken if the attackers obtain the structure and the parameters of the secret part. \emph{An intelligent attacker can eavesdrop on the input-output pairs of the system and estimate the secret part by using system identification methods}. 

Some authors improve their methods for resisting identification. One popular way is periodically switching the parameters of the secret structures, such as in \cite{zhaiSwitchingWatermarkingbasedDetection2021, miaoCodingSchemesSecuring2017,  teixeiraDetectionSensorData2018a}. The auxiliary-system moving target method naturally resists identification because it randomly changes its parameter at each timestamp. Methods in \cite{weerakkodyActiveDetectionExposing2017, miaoCodingSchemesSecuring2017, teixeiraDetectionSensorData2018a} need a pair of synchronized pseudo-random generators to guarantee the parameter matching between the plant side and the controller side. However, the pseudo-random generator may introduce additional risk and may not be adapted to poor network conditions.

In \cite{ferrariSwitchingMultiplicativeWatermarking2021b}, the research proposes a new switching mechanism of multiplicative watermarking. The new mechanism uses an implicit synchronization method and does not need explicitly synchronize components at the controller or plant sides. Researchers in \cite{galloCryptographicSwitchingFunctions2022} transplant the elliptic curve method to further improve the switching function's security.

%% privacy problem
% 1. parameter privacy
% 2. current solution: DP is widely used
% 3. noise-sensitivity
% 4. cryptography:  computation resources

\emph{From another point of view, the problem of designing an unrecognizable secret structure can be regarded as designing a secret structure and protecting the privacy of its parameters}. Privacy of control systems has been another hot topic in recent years \cite{bottegalPreservingPrivacyFinite2017, katewaDifferentialPrivacyNetwork2020, tsiamisStateEstimationCodes2017, tsiamisStateSecrecyCodesStable2018}. Researchers have proposed different methods to protect the state or parameters of control systems from eavesdroppers. 

% Popular solutions 
The differential privacy (DP) method is a popular method to protect the control system's privacy \cite{bottegalPreservingPrivacyFinite2017, katewaDifferentialPrivacyNetwork2020}. However, the fault detection and attack detection scenarios are noise-sensitive. The noise sequence injected in the DP method may increase the false-alarm rate. The higher the privacy level, the higher the false-alarm rate will be introduced. 

Therefore, \emph{how to design a new active detection method or extend existing active detection methods to improve the privacy level of the detection component is still an open question.}

%% possible ways:
% 1. no hardness problem
% 2. but the complex structure
% 3. utilize randomness inherited in dynamical systems instead of pseudo-random
% 4. newly added structure, no noise

In this paper, we aim to design a hybrid multiplicative watermarking method. Compared to the original multiplicative watermarking method, the proposed hybrid multiplicative watermarking method has two modifications:

%% modifications
% 1. improve the detectability:
%    capability to detect control-signal-injection zero-dynamics attack
% 2. improve the structure or the switching rule so that attackers take extra hard to identify the watermarking parameter

\begin{itemize}
    \item Inspired by works in \cite{guoOutputCodingBasedDetectionScheme2021, ghaderiBlendedActiveDetection2021} We improve the detection performance by merging the information of the control signal into the watermarking dynamics;
    \item We propose a new switching method in which the generator and remover select their group of parameters based on their states and input. Furthermore, when generating the parameters of the watermarking components, we design some states to be unobservable. We will prove that this switching method achieves implicit synchronization and does not cause performance loss under normal operation.
\end{itemize}

Compared to other research on active detection methods, we paid more attention to increasing the attacker's difficulty in estimating the private structure. Our main considerations include the following:

% 1. try to use internal noise instead of the attacker cannot know the internal noise sequence, and the process noise is the true random number
% 2. the hardness of identifying the hybrid systems
% 3. the state is driven by the noise; the attacker cannot know the internal noise and the signal affected by the noise()
% 4. introduce an unobservable state that cannot be identified and increase extra hardness to estimate parameters based on input-output pair; we will estimate the in

\begin{itemize}
    \item The difficulty of identification first relates to the hardness of identifying a hybrid system. Identifying a hybrid system requires sufficient data size \cite{} and is an NP-hard problem \cite{}. We will analyze the time and space complexity an attacker needs to estimate the watermarking parameter through input-output pairs. Besides, we will compare the extra time consumption the switching method takes to the attacker and the system.
    \item The state of the watermarking components relates to the parameter selection and is affected by the internal noise of the plant. The noise of a physical process is always a truly random sequence and has a higher security level than a pseudo-random number generator. Without the knowledge of the noise sequence, the attacker cannot access the true value of the signal affected by the noise. We can further design the switching region to be sensitive to noise, leading to an inaccurate attacker estimation. We will provide an example trend to design the switching region and show its performance with simulation.
    \item Theoretically, the dynamics of the introduced unobservable states cannot be identified. Moreover, an unobservable piecewise affine hybrid system cannot be equally modeled by an input-output model \cite{}. However, the unobservable state may decrease the robustness. We will estimate the difficulty the unobservable state takes to the attacker and the robustness of the watermarking method under scenarios such as packet loss or parameter mismatching.
\end{itemize}

% Problem formulation:
% model structure： LTI + controller
% watermarking structure: basic + switching method
% property of watermarking structure: 
%   synchronization: almost hard to lost desynchronization
%   robustness 

% coding
% mwm attack scenarios simulation
% 
